Data Integration Model for Air Quality: A Hierarchical Approach to the Global Estimation of Exposures to Ambient Air Pollution

Air pollution is a major risk factor for global health, with both ambient and household air pollution contributing substantial components of the overall global disease burden. One of the key drivers of adverse health effects is fine particulate matter ambient pollution (PM$_{2.5}$) to which an estimated 3 million deaths can be attributed annually. The primary source of information for estimating exposures has been measurements from ground monitoring networks but, although coverage is increasing, there remain regions in which monitoring is limited. Ground monitoring data therefore needs to be supplemented with information from other sources, such as satellite retrievals of aerosol optical depth and chemical transport models. A hierarchical modelling approach for integrating data from multiple sources is proposed allowing spatially-varying relationships between ground measurements and other factors that estimate air quality. Set within a Bayesian framework, the resulting Data Integration Model for Air Quality (DIMAQ) is used to estimate exposures, together with associated measures of uncertainty, on a high resolution grid covering the entire world. Bayesian analysis on this scale can be computationally challenging and here approximate Bayesian inference is performed using Integrated Nested Laplace Approximations. Model selection and assessment is performed by cross-validation with the final model offering substantial increases in predictive accuracy, particularly in regions where there is sparse ground monitoring, when compared to current approaches: root mean square error (RMSE) reduced from 17.1 to 10.7, and population weighted RMSE from 23.1 to 12.1 $\mu$gm$^{-3}$. Based on summaries of the posterior distributions for each grid cell, it is estimated that 92% of the world's population reside in areas exceeding the World Health Organization's Air Quality Guidelines.

==> Sections/3_modelling_20160817_MLT.tex <==
\section{Statistical Modelling}
The aim of the modelling is to predict concentrations of PM$_{2.5}$ for each of the 1.4 million grid cells, together with associated measures of uncertainty. The general approach is to calibrate ground measurements, where available, with the information from other sources  of information described in Section \ref{sec:data}. The section begins with a brief description of a statistical calibration model and how the relationships between the ground measurements and other variables can be allowed to vary spatially. This is often achieved by assigning random effects to the coefficients of the regression model and assuming that they  arise from a  continuous  spatial process. Here we use a different structure for the model underlying these random effects as, despite  monitoring data being increasingly available, there are  issues that may mean using a spatial continuous process will be problematic. Monitoring protocols,  measurement techniques, quality control procedures and mechanisms for obtaining annual averages may vary from country-to-country \citep{brauer2012exposure} leading to natural discontinuities between countries. In addition to the issues of differing measurement regimes, the geographic distribution of measurements is heavily biased toward North America, Europe, China and India and there are areas of the world, e.g. Africa (as can be seen in Figure \ref{map:gm}) where there  is very little monitoring information to inform such a model.  \\


The structure of the random effects exploits the geographical nested hierarchy within the data: each of the 187 countries in the world are  allocated to one of 21 regions and, further, to one of 7 super-regions. Regions must contain  at least two countries and  are broadly based on geographic regions/sub-continents and groupings based on country level mortality levels and causes of death \citep{brauer2012exposure}. The geographical structure of regions super-regions can be seen in Figure \ref{map:regions}. Although monitoring data is increasingly available, there are  issues that may mean using a spatial continuous process will be problematic. Monitoring protocols,  measurement techniques, quality control procedures and mechanisms for obtaining annual averages may vary from country-to-country \citep{brauer2012exposure} leading to natural discontinuities between countries. In addition to the issues of differing measurement regimes, the geographic distribution of measurements is heavily biased toward North America, Europe, China and India and there are areas of the world, e.g. Africa (as can be seen in Figure \ref{map:gm}) where there  is very little monitoring information to inform such a model. Where there is limited  monitoring data within a country,  information can be borrowed from  higher up  the hierarchy, i.e. from other countries within the region and further, from  the wider super-region.  \\

  \begin{figure}
 \centering
 \begin{subfigure}{\textwidth}  \centering
 \includegraphics[width=0.8\linewidth]{Figures/GBD2015_REGION.png}	
 \caption{Map of regions.}
 \end{subfigure}
  \begin{subfigure}{\textwidth}
 \centering
 \includegraphics[width=0.8\linewidth]{Figures/GBD2015_SREGION.png}	
 \caption{Map of super-regions.}
 \end{subfigure}
 \caption{Schematic showing the nested geographical structure of countries within regions within super-regions. } \label{map:regions}
 \end{figure}  




\subsection{Statistical calibration}

As described in  Section \ref{sec:intro}, in statistical calibration a regression model is used to express the measurements, $Y_s$,  as a function of  covariates, $X_{lr}, r=1,\dots, R$. The measurements, $Y_s$,  are available at a discrete set of $N_S$ locations $S \in \cal{S}$ with  labelling, $S= \{s_0,s_1,\dots,s_{N_S}\}$ whereas the covariates are  available on a grid containing $N_L$  cells, $l \in L$  where $L= l_1, ..., l_{N_L}$. One approach to linking data at different  resolutions is to use spatially varying coefficient models, often referred to as \emph{downscaling} models. For a point, $s$, within grid cell, $X_l$, on which a covariate, $r$, is available,  they  take the form,
\begin{equation} \label{eqn:3}
Y_s = \tilde{\beta}_{0s} + \tilde{\beta}_{1s} X_{lr} + \epsilon_s 
\end{equation}
where $\epsilon_s \sim N(0,\sigma_\epsilon^2)$ is a random error term and 
\begin{eqnarray*}
\tilde{\beta}_{0s} = \beta_0+ \beta_{0s} \\
\tilde{\beta}_{1s} = \beta_1+ \beta_{1s} \; .
\end{eqnarray*}
Here, $\beta_0$ and $\beta_1$ represent the mean value of the additive and multiplicative biases respectively with $\beta_{0s}$ and $\beta_{1s}$ providing localised adjustments to these means. \\

The coefficients, $\beta_{0s}$ and $\beta_{1s}$ are allowed to varying over space, which allows predictions to vary within  grid cells and is the essence of downscaling, in \citet{berrocal2010spatio} for example, $\beta_{0s}$ and $\beta_{1s}$ are modelled as a continuous bivariate spatial process. \\




\subsection{A Data Integration Model for Air Quality}\label{sec:DIMAQ}

Here, ground measurements of $PM_{2.5}$ are available at point locations $s$ within grid cell $l$, country $i$, region $j$  and the super--region $k$  are denoted by $Y_{slijk}$. As described in Section (\ref{sec:data}), there is a nested hierarchical structure with $s=1,\dots, N_l$ sites within grid cell, $l$; $l=1,\dots, N_i$, grid cells within country $i$;  $i=1,\dots, N_j$, countries within region  $j$ and $j=1,\dots, N_k$,  regions  within super--region $k$, $k=1,\dots, N_k$. In order to allow for the  skew in the measurements  and the constraint of non--negativity, the (natural) logarithm of the measurements are modelled as a function of the covariates, $X_1,\dots, X_{10}$.  \\

The model therefore consists of a set of fixed and random effects, for both intercepts and covariates, and is given as follows,
\begin{eqnarray} \label{eqn:arr1} \nonumber
\log(Y_{slijk}) = \beta_0 &+& \sum^{P}_{p=1} \beta_p X_{p,slijk} \\  \nonumber
&+& (\beta_{0l}^G+ \beta_{0i}^C+\beta_{0j}^R+\beta_{0k}^{SR}) \\
&+& \sum_{q \in Q}(\beta_{qi}^C+ \beta_{qj}^R+\beta_{qk}^{SR}) X_{slijk} \\ \nonumber
&+& \epsilon_{slijk} \;.
\end{eqnarray}
Here, the $R$ covariates contain two groups, $R=(P, Q)$ where $P$ are those with  fixed effects and $Q$ those assigned random effects. For the intercept terms, $\beta_{0i}^G$, $\beta_{0i}^C$, $\beta_{0j}^R$ and $\beta_{0k}^{SR}$ represent the coefficients for grid cell $l$, country $i$ within region $j$ and super--region $k$. For the covariate effects, the notation is the same but there is no grid cell effect, e.g.  $\beta_{qi}^C$, $\beta_{qj}^R$ and $\beta_{qk}^{SR}$ represent country, region and super--region effects respectively. The term $\epsilon_{slijk}$ denotes random error term with $\epsilon_{slijk} \sim N(0, \sigma^2_{\epsilon})$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Structure of the random effects}

Equation (\ref{eqn:arr1}) can be expressed in a similar form to that seen in Equation (\ref{eqn:3}),
\begin{eqnarray} \label{eqn:arr1} \nonumber
\log(Y_{slijk}) = \tilde{\beta}_{0,lijk} &+& \sum_{q \in Q} \tilde{\beta}_{q, ijk} X_{q,slijk} \\ \nonumber 
&+& \sum_{p \notin Q} \beta_p X_{p,slijk}  \\
&+& \epsilon_{slijk} \;, 
\end{eqnarray}
where $\epsilon_{slijk} \sim N(0,\sigma_{\epsilon}^2)$ is a random error term. \\

Here,  the random effect terms, $\tilde{\beta}_{0,lijk}$ and $\tilde{\beta}_{1,ijk}$ have contributions from the cell (in the case of the intercept), the country, the region and the super--region as follows, 
\begin{eqnarray}
\tilde{\beta}_{0, lijk} = \beta_0+ \beta_{0,l}^G + \beta_{0,i}^C + \beta_{0,j}^R +\beta_{0,k}^{SR} \\
\tilde{\beta}_{q, lijk} = \beta_q+  \beta_{q,i}^C + \beta_{q,j}^R +\beta_{q,k}^{SR} \; .
\end{eqnarray}
For clarity of exposition, we restrict the following description to a generic parameter, $\beta$. Let $\beta^{SR}_k$ denote the coefficient for  super-region $k$. The coefficients for super-regions  are distributed with mean equal to the overall mean ($\beta_0$, the fixed effect) and variance representing between super-region variability,
\begin{equation*}
\beta^{SR}_{k} \sim N(\beta_0,\sigma_{SR}^2) \,
\end{equation*}
where $k=1,\ldots,N_k = 7$. Similarly, each super-region contains a number of regions. Let $\beta^{R}_{j}$ denote the coefficient for region $j$ which will be distributed with mean equal to to the coefficient for the  super-region $k$ that contains region $j$ and variance representing the between region (within super--region) variability. 
\begin{equation*}
\beta^{R}_{j} \sim N(\beta^{SR}_k,\sigma^2_{R,l}) 
\end{equation*}
where $j=1,\ldots,N_k$,  the number of regions in super-region $j$. Each region will itself, contain a number of countries. Let $\beta^{C}_{ijk}$ denote the coefficient for  country $i$ in region $j$ and super-region $k$. The country level effect will be distributed with mean equal  to the coefficient for region $j$ within super-region $k$ with variance representing  the between country (within region) variability.
\begin{equation} \label{eqn:countr1}
\beta^{C}_{i} \sim N(\beta^{R}_{j},\sigma^2_{C, j})
\end{equation}
where $j=1,\ldots,N_j$ is   the number of countries in region $k$. Note that in the case of the intercepts, there is an additional term, $\beta^G_{l}$,  representing between location, within grid cell, variability. \\

Here, super--region effects, regional effects within super--regions and country effects within regions are assumed to be independent and identically distributed. The geographical hierarchy is broadly based on geographic regions, sub-continents, mortality and economic factors \citep{brauer2012exposure}. As such, there are countries for which the allocation may not be optimal  when considering environmental factors, such as air pollution. For example, Mongolia is part of the Asia Central region and Central Eastern Europe and Central Asia super--region (see Figure \ref{map:regions}) whereas it might be expected to have features more akin to its more direct neighbours, rather than more western countries, including China which is in a different region (Asia East) and super--region (South East Asia, East Asia and Oceania). For this reason, it might be advantageous to restrict the borrowing of information in Equation (\ref{eqn:countr1}) to a countries immediate neighbours rather than all of the countries in its administrative region. This could be achieved using a ICAR model \citep{besag1974spatial}, 
\begin{equation} \label{eqn:countr2}
\beta^{C}_{i} | \beta^{C}_{i'}, \; i' \in \partial_i \sim N\left(
  \overline{\beta}^{C}_{i},\frac{\psi^2}{N_{\partial i}}\right),
  \end{equation}
where $\partial i$ is the set of neighbours of country $i$, $N_{\partial i}$ is the number of neighbours, and $\overline{\beta}^{C}_i$ is the mean of the spatial random effects of these neighbours.

\subsection{Inference}


The model presented here is a Bayesian hierarchical model with three levels: (i) the data, or observation level; (ii) the process, or parameter, level and (iii)  the hyperparameter level. 

\begin{eqnarray} \label{eqn:lgm1} \nonumber
Y|\theta, \psi &\sim& \prod^{N_S}_{s} p(Y_s| \theta, \psi)\\  \nonumber
\theta | \psi &\sim & p(\theta | \psi)\\
\psi &\sim& p(\psi)
\end{eqnarray}
where $\theta$ are the parameters of the model as described in Section \ref{sec:DIMAQ}. Here,  $\theta = (\beta_0+ \beta_{0,l}^G + \beta_{0,i}^C + \beta_{0,j}^R +\beta_{0,k}^{SR}, \beta_q+  \beta_{q,i}^C + \beta_{q,j}^R +\beta_{q,k}^{SR})$. The set of hyperparameters, $\psi$, contain those at both the first, $\psi_1$, and second, $\psi_2$ levels of the model, $\psi=(\psi_1, \psi_2)$, where $\psi_1=(\sigma^2_{\epsilon})$ and $\psi_2=(\sigma^2_{G,i},\sigma^2_{C,j}, \sigma^2_{R,j}, \sigma^2_{SR})$. \\

The model is implemented using approximate Bayesian inference using integrated nested Laplace Approximations (INLA) proposed in\citet{rue2009approximate} using the R-INLA software \citep{rue2012r}. This can be applied to models that can be expressed as a latent Gaussian model (LGM) and has been developed as a computationally attractive alternative to MCMC. \\


\subsubsection{Latent Gaussian models}
If a model can be expressed in terms of a latent Gaussian model than we can take advantage of features that can facilitate efficient computation. Latent Gaussian models  are a general class of models and allow a very wide range of formulations.  Given $\eta_s = g(E(Y_s))$, the general form  of a LGM is

\begin{eqnarray}
\eta_s &=& \beta_0 + \sum_{p=1}^{P} \beta_p X_{qs} + \sum^Q_{q=1} f_q (Z_{qs}) 	
\end{eqnarray}
where $\beta_0$ is an overall intercept term, the set of $\beta_p$ $(p=1,\dots, P)$ are the coefficients associated with covariates, $X$; the fixed effects. The set of functions,  $f_1(\cdot), \dots, f_Q(\cdot)$ represent the random effects withe the form of the function being determined by the model. For example a hierarchical model may have, $f_1(\cdot) \sim N(0, \sigma^2_f)$, with a distribution defined for $\sigma^2_f| \psi$, whereas for standard regression, $f(\cdot)=0$, leaving just fixed effects. \\

In this case, the set of unknown parameters, $\theta$, will include both the coefficients of the model and the parameters required for the functions, i.e. $\theta = (\beta, f)$. For a LGM, the collection of all of these parameters will be assigned a Normal distributed  in the second level of the model shown in Equation (\ref{eqn:lgm1}), e.g. $\theta | \psi \sim  MVN(\theta | \Sigma(\psi_2))$. If this can be expressed in terms of a GMRF then it may be possible to take advantage of methods that reduced computation in performing Bayesian analysis on models of this type \citep{rue2005gaussian}. \\

The computation required to perform inference on a LGM will be largely determined by the characteristics of the covariance matrix, $\Sigma (\psi_2)$. This will often be dense, i.e. it will have many entries that are non-zero, which commonly leads to a high computational burden when performing  the matrix inversions that will be required to perform inference. Using a GMRF means that   typically  the inverse of the covariance matrix, $Q = \Sigma^{-1}$ will be sparse, i.e. more zero entries,  due to the conditional independence between sets of parameters in which $\theta_l \ci  \theta_m | \theta_{-lm} \iff Q_{lm}=0$ (where $-lm$ denotes the vector of $\theta$ with the $l$ and $m$ elements removed) \citep{rue2005gaussian}. \\

The second level of the model shown in Equation (\ref{eqn:lgm1}) is therefore now expressed as, $\theta | \psi \sim  MVN(\theta | Q(\psi_2)^{-1}$), where  $\psi_2$  denotes the parameters associated with $Q$ rather than $\Sigma$. \\

\subsubsection{Integrated Laplace Approximations}

Estimation of the (marginal) distributions of the model parameters and hyperparameters of the LGM shown in Equation (\ref{eqn:lgm1}) will require evaluation of the following integrals:

\begin{eqnarray} \nonumber \label{eqn:lgm2}
	p(\theta_j | Y) &=& \int p(\theta_j | Y, \psi)p(\psi|Y) d \psi \\ 
		p(\psi_k | Y) &=& \int p(\psi | Y) d \psi_{-k}
\end{eqnarray}

In all but the most stylised cases, these will not be analytically tractable. Samples from these distributions could be obtained using Markov-chain Monte Carlo methods. However there may be issues when fitting complex LGMs and the computational burden may be excessive, especially large numbers of predictions are required, as is the case here. Here we make use of  techniques that perform ‘approximate’ Bayesian inference based on integrated nested Laplace approximations (INLA) that do not require full MCMC sampling to be performed.  It is noted that the dimension of $\theta$ is much larger than the dimension of $\psi$ and feature  LGMs will help in the implementation of the model as the computational burden increases linearly with the dimension of $\theta$ but exponentially with the dimension of $\psi$.\\



The aim is to find approximations for the distributions shown in Equation (\ref{eqn:lgm2}).  For the hyperparameters, the posterior of $\psi$ given $Y$ can be written as

\begin{eqnarray} \nonumber
p(\psi|Y) &=& \frac{p(\theta,\psi| Y)}{p(\theta| \psi, Y)} \\ \nonumber
&\propto & \frac{p(Y|\theta)p(\theta|\psi)p(\psi)}{p(\theta|\psi, Y)} \\  \nonumber
&\approx & \left.\frac{p(Y|\theta)(\theta|\psi)p(\psi)}{\tilde{p}(\theta|\psi, Y)} \right| _{\theta = \hat{\theta}(\psi)} \\ 
&=& \tilde{p}(\psi | Y)\; .
\end{eqnarray}
Here a Laplace approximation (LA) is used in the denominator for $\tilde{p}(\theta|\psi, Y)$. For univariate $\theta$ with an integral of the form $\int e^{g(\theta)}$, the LA takes the form $g(\theta) \sim N(\hat{\theta}(\psi), \hat{\sigma}^2)$, where $\hat{\theta}(\psi)$ is the modal value of $\theta$ for specific values of the hyperparameters, $\psi$ and $\hat{\sigma}^2 = \left\{ \frac{d^2 \log g(\theta)}{d \theta^2} \right \}^{-1}$. \\

The mode of $\tilde{p}(\psi | Y)$ can be found by Newton type algorithms. Around the mode, the  distribution, $\log \tilde{p} (\psi | Y)$, is evaluated over a grid of $H$ points,  $\{\psi*_h\}$, with  associated integration weights $\Delta_k$.   on a grid the marginal posterior, $\tilde{p}(\psi_k | Y)$ is obtained. Once $\tilde{p}(\psi |Y)$ is found, approximations to the marginal distributions, $p(\psi_k |Y)$, can be found using numerical integration. \\


For the model individual model parameters, $\theta_j$,

\begin{eqnarray} \nonumber
p(\theta_j|Y) &=& \frac{p((\theta_j, \theta_{-j}),\psi| Y)}{p(\theta_{-j}| \theta_{j}, \psi, Y)} \\ \nonumber
&\propto & \frac{p(Y|\theta)p(\theta|\psi)p(\psi)}{p(\theta_{-j}| \theta_{j}, \psi, Y)}\\ 
&\approx & \left.\frac{p(Y|\theta)(\theta|\psi)p(\psi)}{\tilde{p}(\theta_{-j}| \theta_{j}, \psi, Y)} \right| _{\theta_{-j} = \hat{\theta_{-j}}(\theta_{j}, \psi)} \\ \nonumber
&=& \tilde{p}(\theta_j | \psi, Y)\; .
\end{eqnarray}

When using a LGM, $(\theta_{-j}| \theta_{j}, \psi, Y)$ will be approximately Gaussian. There are a number of ways of constructing the approximation in the denominator including a simple Gaussian approximation which will be   computationally attractive but may be inaccurate. Alternatively, a LA would be  highly accurate but computationally expensive. R-INLA uses a computationally efficient method, a simplified LA, that consists of performing a Taylor expansion around the LA of $\tilde{p}(\theta_j|\psi, Y)$, aiming to
`correct' the Gaussian approximation for location and
skewness.\\

Numerically, $\tilde{p}(\theta_j | \psi_k, Y)$ is evaluated over a grid with $\tilde{p}(\theta_j |  Y)$ being obtained using numerical integration, $\tilde{p}(\theta_j |  Y) = \sum^H_k = \tilde{p}(\theta_j | \psi^*_k, Y)\tilde{p}(\psi^*_h|Y) \Delta_h$. As the grid takes the form of a regular lattice,  the integration weights, $\Delta_h$ will be equal in this case. \\

The model presented in Section \ref{sec:DIMAQ}  was implemented using  R-INLA  \citep{rue2012r} using the Balena high performance computing system (HPC) at the the University of Bath (www.bath.ac.uk/bucs/services/hpc/facilities/). INLA requires a copy of the model to be stored on a single  node which,  even with high-memory compute nodes (32GBs per core), resulted in memory issues when attempting to perform estimation and prediction on the entire grid of 1.4 million cells in one step. Therefore, an iterative approach to prediction was used, repeatedly appending subsets of the prediction grid (with associated data on satellite estimates and other predictors)  to the modelling dataset,  until a complete set of global predictions  were obtained.



==> Sections/3_modelling_20160818_GS.tex <==
\section{Statistical Modelling} \label{sec:statsmod}
The aim  is to obtain predict concentrations of PM$_{2.5}$ for each of  1.4 million grid cells, together with associated measures of uncertainty. This will be achieved by finding the posterior distributions for each cell, from which summary measures will be calculated. The overall approach is calibration as described in  \citet{chang2016}:  a regression model is used to express ground measurements, $Y_s$, (where available)  as a function of covariates, $X_{lr}$: $r=1,\dots, R$, that reflect the information from other sources  that may  either effect air quality or the accuracy of the measurements,  as described in Section \ref{sec:data}. \\

In statistical calibration, measurements, $Y_s$,  are available at a discrete set of $N_S$ locations $S \in \cal{S}$ with  labelling, $S= \{s_0,s_1,\dots,s_{N_S}\}$ whereas the covariates may be  available on a grid containing $N_L$  cells, $l \in L$  where $L= l_1, ..., l_{N_L}$. One approach to linking data at different  resolutions is to use spatially varying coefficient models, often referred to as \emph{downscaling} models. For a point, $s$, within grid cell, $X_l$, on which a covariate, $r$, is available,  they  take the form,
\begin{equation} \label{eqn:3}
Y_s = \tilde{\beta}_{0s} + \tilde{\beta}_{1s} X_{lr} + \epsilon_s 
\end{equation}
where $\epsilon_s \sim N(0,\sigma_\epsilon^2)$ is a random error term and 
\begin{eqnarray*}
\tilde{\beta}_{0s} = \beta_0+ \beta_{0s} \\
\tilde{\beta}_{1s} = \beta_1+ \beta_{1s} \; .
\end{eqnarray*}
Here, $\beta_0$ and $\beta_1$ represent the mean value of the intercept and coefficients respectively with  providing (spatially driven) adjustments to these means. Allowing $\beta_{0s}$ and $\beta_{1s}$ to vary spatially  is often achieved by assigning random effects to the coefficients of the regression model and assuming that they  arise from a  continuous  spatial process, in \citet{berrocal2010spatio} for example,  $\beta_{0s}$ and $\beta_{1s}$  are assumed to arise from  a continuous bivariate spatial process. \\

Here we consider a different structure for the model underlying these random effects as, despite  monitoring data being increasingly available, there are  issues that may mean using a spatial continuous process will be problematic. Monitoring protocols,  measurement techniques, quality control procedures and mechanisms for obtaining annual averages may vary from country-to-country \citep{brauer2012exposure} leading to natural discontinuities between countries. In addition to the issues of differing measurement regimes, the geographic distribution of measurements is heavily biased toward North America, Europe, China and India and there are areas of the world, e.g. Africa,  as can be seen in Figure \ref{map:gm}, where there  is very little monitoring information to inform such a model.  \\


The structure of the random effects used here exploits the geographical nested hierarchy within the data: each of the 187 countries in the world are  allocated to one of 21 regions and, further, to one of 7 super-regions. Regions must contain  at least two countries and  are broadly based on geographic regions/sub-continents and groupings based on country level mortality levels and causes of death \citep{brauer2012exposure}. The geographical structure of regions super-regions can be seen in Figure \ref{map:regions}. Where there is limited  monitoring data within a country,  information can be borrowed from  higher up  the hierarchy, i.e. from other countries within the region and further, from  the wider super-region.  \\

  \begin{figure}
 \centering
 \begin{subfigure}{\textwidth}  \centering
 \includegraphics[width=0.8\linewidth]{Figures/GBD2015_REGION.png}	
 \caption{Map of regions.}
 \end{subfigure}
  \begin{subfigure}{\textwidth}
 \centering
 \includegraphics[width=0.8\linewidth]{Figures/GBD2015_SREGION.png}	
 \caption{Map of super-regions.}
 \end{subfigure}
 \caption{Schematic showing the nested geographical structure of countries within regions within super-regions. } \label{map:regions}
 \end{figure}  


\subsection{A Data Integration Model for Air Quality}\label{sec:DIMAQ}

Ground measurements  at point locations, $s$, within grid cell, $l$, country, $i$, region, $j$,  and  super--region, $k$  are denoted by $Y_{slijk}$. As described in Section \ref{sec:statsmod}, there is a nested hierarchical structure with $s=1,\dots, N_l$ sites within grid cell, $l$: $l=1,\dots, N_i$, grid cells within country $i$;  $i=1,\dots, N_j$, countries within region  $j$: $j=1,\dots, N_k$,  regions  within super--region $k$: $k=1,\dots, N_k$. In order to allow for the  skew in the measurements  and the constraint of non--negativity, the (natural) logarithm of the measurements are modelled as a function of the covariates, $X_{lr}$: $r=1,\dots, R$.  \\



The model  consists of a set of fixed and random effects, for both intercepts and covariates, and is given as follows,
\begin{eqnarray} \label{eqn:arr1} \nonumber
\log(Y_{slijk}) = \beta_0 &+& \sum^{P}_{p=1} \beta_p X_{p,slijk} \\  \nonumber
&+& (\beta_{0l}^G+ \beta_{0i}^C+\beta_{0j}^R+\beta_{0k}^{SR}) \\
&+& \sum_{q \in Q}(\beta_{qi}^C+ \beta_{qj}^R+\beta_{qk}^{SR}) X_{slijk} \\ \nonumber
&+& \epsilon_{slijk} \;.
\end{eqnarray}
Here, the set of $R$ covariates consists of two groups, $R=(P, Q)$ where $P$ are those with just  fixed effects and $Q$ those additionally assigned random effects. For the intercept terms: $\beta_{0i}^G$, $\beta_{0i}^C$, $\beta_{0j}^R$ and $\beta_{0k}^{SR}$ represent the coefficients for grid cell $l$, country $i$ within region $j$ and super--region $k$. For the covariate effects, the notation is the same but there is no grid cell effect, with  $\beta_{qi}^C$, $\beta_{qj}^R$ and $\beta_{qk}^{SR}$ representing country, region and super--region effects respectively. The term $\epsilon_{slijk}$ denotes random error term with $\epsilon_{slijk} \sim N(0, \sigma^2_{\epsilon})$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Structure of the random effects}

Equation (\ref{eqn:arr1}) can be expressed in a similar form to that seen in Equation (\ref{eqn:3}),
\begin{eqnarray} \label{eqn:arr1} \nonumber
\log(Y_{slijk}) = \tilde{\beta}_{0,lijk} &+& \sum_{q \in Q} \tilde{\beta}_{q, ijk} X_{q,slijk} \\ \nonumber 
&+& \sum_{p \notin Q} \beta_p X_{p,slijk}  \\
&+& \epsilon_{slijk} \;, 
\end{eqnarray}
where $\epsilon_{slijk} \sim N(0,\sigma_{\epsilon}^2)$ is a random error term. \\

Here,  the random effect terms, $\tilde{\beta}_{0,lijk}$ and $\tilde{\beta}_{1,ijk}$, have contributions from  the country, the region and the super--region, with the intercept also having a random effect for the cell representing within-cell variation in ground measurements,  
\begin{eqnarray}
\tilde{\beta}_{0, lijk} = \beta_0+ \beta_{0,l}^G + \beta_{0,i}^C + \beta_{0,j}^R +\beta_{0,k}^{SR} \\
\tilde{\beta}_{q, lijk} = \beta_q+  \beta_{q,i}^C + \beta_{q,j}^R +\beta_{q,k}^{SR} \; .
\end{eqnarray}
For clarity of exposition, we restrict the following description to a generic parameter, $\beta$. Let $\beta^{SR}_k$ denote the coefficient for  super-region $k$. The coefficients for super-regions  are distributed with mean equal to the overall mean ($\beta_0$, the fixed effect) and variance representing between super-region variability,
\begin{equation*}
\beta^{SR}_{k} \sim N(\beta_0,\sigma_{SR}^2) \,
\end{equation*}
where $k=1,\ldots,N_k = 7$. Similarly, each super-region contains a number of regions. Let $\beta^{R}_{j}$ denote the coefficient for region $j$ which will be distributed with mean equal to to the coefficient for the  super-region $k$ that contains region $j$ and variance representing the between region (within super--region) variability. 
\begin{equation*}
\beta^{R}_{j} \sim N(\beta^{SR}_k,\sigma^2_{R,l}) 
\end{equation*}
where $j=1,\ldots,N_k$,  the number of regions in super-region $j$. Each region will itself, contain a number of countries. Let $\beta^{C}_{ijk}$ denote the coefficient for  country $i$ in region $j$ and super-region $k$. The country level effect will be distributed with mean equal  to the coefficient for region $j$ within super-region $k$ with variance representing  the between country (within region) variability.
\begin{equation} \label{eqn:countr1}
\beta^{C}_{i} \sim N(\beta^{R}_{j},\sigma^2_{C, j})
\end{equation}
where $j=1,\ldots,N_j$ is   the number of countries in region $k$. Note that in the case of the intercepts, there is an additional term, $\beta^G_{l}$,  representing between location, within grid cell, variability. \\

Country effects within regions and regional effects within super--regions  are assumed to be independent  within their respective geographies. However, the geographical hierarchy is broadly based on geographic regions, sub-continents, mortality and economic factors \citep{brauer2012exposure} and, as such, there are countries for which the allocation may not be optimal  when considering environmental factors, such as air pollution. For example, Mongolia is part of the Asia Central region and Central Eastern Europe and Central Asia super--region (see Figure \ref{map:regions}) but it's pollution profile might be expected to be more similar to its more direct neighbours, including China  (which is in a different region (Asia East) and super--region (South East Asia, East Asia and Oceania)), rather than more western countries. For this reason, it might be advantageous to allow the borrowing of information in Equation (\ref{eqn:countr1}) to inlcude countries that are immediate neighbours rather than all of the countries in the surrounding administrative region. This could be achieved using a conditionally autoregressive (ICAR) model \citep{besag1974spatial} in place of Equation (\ref{eqn:countr1}), 
\begin{equation} \label{eqn:countr2}
\beta^{C}_{i} | \beta^{C}_{i'}, \; i' \in \partial_i \sim N\left(
  \overline{\beta}^{C}_{i},\frac{\psi^2}{N_{\partial i}}\right),
  \end{equation}
where $\partial i$ is the set of neighbours of country $i$, $N_{\partial i}$ is the number of neighbours, and $\overline{\beta}^{C}_i$ is the mean of the spatial random effects of these neighbours.

\subsection{Inference}
The model is implemented using approximate Bayesian inference using integrated nested Laplace Approximations (INLA) proposed in \citet{rue2009approximate} using the R-INLA software \citep{rue2012r}. This can be applied to models that can be expressed as a latent Gaussian model (LGM). The model is a Bayesian hierarchical model with three levels: (i) the data, or observation level; (ii) the process, or parameter, level and (iii)  the hyperparameter level. 

\begin{eqnarray} \label{eqn:lgm1} \nonumber
Y|\theta, \psi &\sim& \prod^{N_S}_{s} p(Y_s| \theta, \psi)\\  \nonumber
\theta | \psi &\sim & p(\theta | \psi)\\
\psi &\sim& p(\psi)
\end{eqnarray}
where $\theta$ are the parameters of the model as described in Section \ref{sec:DIMAQ} and will include $\beta_0+ \beta_{0,l}^G + \beta_{0,i}^C + \beta_{0,j}^R +\beta_{0,k}^{SR}, \beta_q+  \beta_{q,i}^C + \beta_{q,j}^R +\beta_{q,k}^{SR})$. The set of hyperparameters, $\psi$, contain those at both the first, $\psi_1$, and second, $\psi_2$ levels of the model, $\psi=(\psi_1, \psi_2)$, where $\psi_1=(\sigma^2_{\epsilon})$ and $\psi_2=(\sigma^2_{G,i},\sigma^2_{C,j}, \sigma^2_{R,j}, \sigma^2_{SR})$. \\




\subsubsection{Latent Gaussian models}
The model can be expressed in terms of a LGM meaning that we can take advantage of features that can facilitate efficient computation. LGMs  are a general class of models and allow a very wide range of formulations.  Given $\eta_s = g(E(Y_s))$, the general form  of a LGM is

\begin{eqnarray}
\eta_s &=& \beta_0 + \sum_{p=1}^{P} \beta_p X_{qs} + \sum^Q_{q=1} f_q (Z_{qs}) 	
\end{eqnarray}
where $\beta_0$ is an overall intercept term, the set of $\beta_p$ $(p=1,\dots, P)$ are the coefficients associated with covariates, $X$; the fixed effects. The set of functions,  $f_1(\cdot), \dots, f_Q(\cdot)$ represent the random effects withe the form of the function being determined by the model. For example a hierarchical model may have, $f_1(\cdot) \sim N(0, \sigma^2_f)$, with a distribution defined for $\sigma^2_f| \psi$, whereas for standard regression, $f(\cdot)=0$, leaving just fixed effects. \\

The set of unknown parameters, $\theta$, will include both the coefficients of the model shown above and the parameters required for the functions, i.e. $\theta = (\beta, f)$. For a LGM, the collection of all of these parameters will be assigned a Normal distributed  in the second level of the model shown in Equation (\ref{eqn:lgm1}), e.g. $\theta | \psi \sim  MVN(\theta | \Sigma(\psi_2))$. The computation required to perform inference on a LGM will be largely determined by the characteristics of the covariance matrix, $\Sigma (\psi_2)$. This will often be dense, i.e. it will have many entries that are non-zero, which commonly leads to a high computational burden when performing  the matrix inversions that will be required to perform inference. \\

If  $\theta | \psi$ can be expressed in terms of a Gaussian Markov Random Field (GMRF),  then it may be possible to take advantage of methods that reduced computation in performing Bayesian analysis on models of this type \citep{rue2005gaussian}. Using a GMRF means that   typically  the inverse of the covariance matrix, $Q = \Sigma^{-1}$ will be sparse, i.e. more zero entries,  due to the conditional independence between sets of parameters in which $\theta_l \ci  \theta_m | \theta_{-lm} \iff Q_{lm}=0$ (where $-lm$ denotes the vector of $\theta$ with the $l$ and $m$ elements removed) \citep{rue2005gaussian}. Assuming that  $\theta | \psi \sim GMRF$ then the second level of the model shown in Equation (\ref{eqn:lgm1}) is therefore now expressed as, $\theta | \psi \sim  MVN(\theta | Q(\psi_2)^{-1}$), where  $\psi_2$  denotes the parameters associated with $Q$ rather than $\Sigma$. \\

\subsubsection{Integrated Laplace Approximations}

Estimation of the (marginal) distributions of the model parameters and hyperparameters of the LGM shown in Equation (\ref{eqn:lgm1}) will require evaluation of the following integrals:

\begin{eqnarray} \nonumber \label{eqn:lgm2}
	p(\theta_j | Y) &=& \int p(\theta_j | Y, \psi)p(\psi|Y) d \psi \\ 
		p(\psi_k | Y) &=& \int p(\psi | Y) d \psi_{-k}
\end{eqnarray}

In all but the most stylised cases, these will not be analytically tractable. Samples from these distributions could be obtained using Markov-chain Monte Carlo methods but  there may be issues when fitting complex LGMs and the computational burden may be excessive, especially large numbers of predictions are required.   Here,   approximate Bayesian inference is performed  based on integrated nested Laplace approximations (INLA). It is noted that the dimension of $\theta$ is much larger than the dimension of $\psi$ and this will help in the implementation of the model as the computational burden increases linearly with the dimension of $\theta$ but exponentially with the dimension of $\psi$.\\



The aim is to find approximations for the distributions shown in Equation (\ref{eqn:lgm2}).  For the hyperparameters, the posterior of $\psi$ given $Y$ can be written as

\begin{eqnarray} \nonumber
p(\psi|Y) &=& \frac{p(\theta,\psi| Y)}{p(\theta| \psi, Y)} \\ \nonumber
&\propto & \frac{p(Y|\theta)p(\theta|\psi)p(\psi)}{p(\theta|\psi, Y)} \\  \nonumber
&\approx & \left.\frac{p(Y|\theta)(\theta|\psi)p(\psi)}{\tilde{p}(\theta|\psi, Y)} \right| _{\theta = \hat{\theta}(\psi)} \\ 
&=& \tilde{p}(\psi | Y)\; .
\end{eqnarray}
Here a Laplace approximation (LA) is used in the denominator for $\tilde{p}(\theta|\psi, Y)$. For univariate $\theta$ with an integral of the form $\int e^{g(\theta)}$, the LA takes the form $g(\theta) \sim N(\hat{\theta}(\psi), \hat{\sigma}^2)$, where $\hat{\theta}(\psi)$ is the modal value of $\theta$ for specific values of the hyperparameters, $\psi$ and $\hat{\sigma}^2 = \left\{ \frac{d^2 \log g(\theta)}{d \theta^2} \right \}^{-1}$. \\

The mode of $\tilde{p}(\psi | Y)$ can be found by Newton type algorithms. Around the mode, the  distribution, $\log \tilde{p} (\psi | Y)$, is evaluated over a grid of $H$ points,  $\{\psi*_h\}$, with  associated integration weights $\Delta_k$.   on a grid the marginal posterior, $\tilde{p}(\psi_k | Y)$ is obtained. Once $\tilde{p}(\psi |Y)$ is found, approximations to the marginal distributions, $p(\psi_k |Y)$, can be found using numerical integration. \\


For the model individual model parameters, $\theta_j$,

\begin{eqnarray} \nonumber
p(\theta_j|Y) &=& \frac{p((\theta_j, \theta_{-j}),\psi| Y)}{p(\theta_{-j}| \theta_{j}, \psi, Y)} \\ \nonumber
&\propto & \frac{p(Y|\theta)p(\theta|\psi)p(\psi)}{p(\theta_{-j}| \theta_{j}, \psi, Y)}\\ 
&\approx & \left.\frac{p(Y|\theta)(\theta|\psi)p(\psi)}{\tilde{p}(\theta_{-j}| \theta_{j}, \psi, Y)} \right| _{\theta_{-j} = \hat{\theta_{-j}}(\theta_{j}, \psi)} \\ \nonumber
&=& \tilde{p}(\theta_j | \psi, Y)\; .
\end{eqnarray}

For a LGM, $(\theta_{-j}| \theta_{j}, \psi, Y)$ will be approximately Gaussian. There are a number of ways of constructing the approximation in the denominator including a simple Gaussian approximation which will be   computationally attractive but may be inaccurate. Alternatively, a LA would be  highly accurate but computationally expensive. R-INLA uses a computationally efficient method, a simplified LA, that consists of performing a Taylor expansion around the LA of $\tilde{p}(\theta_j|\psi, Y)$, aiming to
`correct' the Gaussian approximation for location and
skewness.\\

Numerically, $\tilde{p}(\theta_j | \psi_k, Y)$ is evaluated over a grid with $\tilde{p}(\theta_j |  Y)$ being obtained using numerical integration, $\tilde{p}(\theta_j |  Y) = \sum^H_k = \tilde{p}(\theta_j | \psi^*_k, Y)\tilde{p}(\psi^*_h|Y) \Delta_h$. When the grid takes the form of a regular lattice,  the integration weights, $\Delta_h$ will be equal. \\

The model presented in Section \ref{sec:DIMAQ}  was implemented using  R-INLA  \citep{rue2012r} using the Balena high performance computing system (HPC) at the the University of Bath \newline \verb (www.bath.ac.uk/bucs/services/hpc/facilities/).   INLA requires a copy of the model to be stored on a single  node which,  even with high-memory compute nodes (32GBs per core), resulted in memory issues when attempting to perform estimation and prediction on the entire grid of 1.4 million cells in one step. Therefore, an iterative approach to prediction was used, repeatedly appending subsets of the prediction grid (with associated data on satellite estimates and other predictors)  to the modelling dataset,  until a complete set of global predictions  were obtained.



==> Sections/3_modelling_20160818_GS2.tex <==
\section{Statistical Modelling} \label{sec:statsmod}
The aim  is to obtain predict concentrations of PM$_{2.5}$ for each of  1.4 million grid cells, together with associated measures of uncertainty. This will be achieved by finding the posterior distributions for each cell, from which summary measures will be calculated. \\


The overall approach is statistical calibration as described in  \citet{chang2016}:  a regression model is used to express ground measurements, $Y_s$,   available at a discrete set of $N_S$ locations $S \in \cal{S}$ with  labelling, $S= \{s_0,s_1,\dots,s_{N_S}\}$  as a function of covariates, $X_{sr}$: $r=1,\dots, R$, that reflect  information from other sources,  as described in Section \ref{sec:data}. Covariate information may be available for point locations (as with the ground measurements)  or on a grid of $N_L$  cells, $l \in L$  where $L= l_1, ..., l_{N_L}$. Considering a single covariate, $X_{lr}$, measured on a grid, 


\begin{equation} \label{eqn:3}
Y_s = \tilde{\beta}_{0s} + \tilde{\beta}_{1s} X_{lr} + \epsilon_s 
\end{equation}
where $\epsilon_s \sim N(0,\sigma_\epsilon^2)$ is a random error term. The terms $\tilde{\beta}_{0s}$ and $\tilde{\beta}_{1s}$ denote random effects that allow the intercept and coefficient to vary over space
\begin{eqnarray*}
\tilde{\beta}_{0s} = \beta_0+ \beta_{0s} \\
\tilde{\beta}_{1s} = \beta_1+ \beta_{1s} \; .
\end{eqnarray*}
Here, $\beta_0$ and $\beta_1$ represent the mean value of the intercept and coefficients respectively with $\beta_{0s}$ and $\beta_{1s}$ providing (spatially driven) adjustments to these means, allowing the calibration functions to vary over space. In downscaling models, it is assumed that the parameters $\beta_{0s}$ and $\beta_{1s}$ arise from a  continuous  spatial process which allows with grid-cell variation (see \citet{berrocal2010spatio} for an example using a continuous bivariate spatial process). \\


Despite  monitoring data being increasingly available, there are  issues that may mean using a spatial continuous process may be problematic in this setting. Monitoring protocols,  measurement techniques, quality control procedures and mechanisms for obtaining annual averages may vary from country-to-country \citep{brauer2012exposure} leading to natural discontinuities (in ground measurements) between countries. In addition, the geographic distribution of measurements is heavily biased toward North America, Europe, China and India and there are areas of the world, e.g. Africa,  as can be seen in Figure \ref{map:gm}, where there  will be very little monitoring information to inform such a model.  \\


The structure of the random effects used here exploits a geographical nested hierarchy: each of the 187 countries considered are  allocated to one of 21 regions and, further, to one of 7 super-regions. Each region must contain  at least two countries and  is broadly based on geographic regions/sub-continents and groupings based on country level development status and causes of death \citep{brauer2012exposure}. The geographical structure of regions within super-regions can be seen in Figure \ref{map:regions}. Where there is limited  monitoring data within a country,  information can be borrowed from  higher up  the hierarchy, i.e. from other countries within the region and further, from  the wider super-region.  \\

  \begin{figure}
 \centering
 \begin{subfigure}{\textwidth}  \centering
 \includegraphics[width=0.8\linewidth]{Figures/GBD2015_REGION.png}	
 \caption{Map of regions.}
 \end{subfigure}
  \begin{subfigure}{\textwidth}
 \centering
 \includegraphics[width=0.8\linewidth]{Figures/GBD2015_SREGION.png}	
 \caption{Map of super-regions.}
 \end{subfigure}
 \caption{Schematic showing the nested geographical structure of countries within regions within super-regions. } \label{map:regions}
 \end{figure}  


\subsection{A Data Integration Model for Air Quality}\label{sec:DIMAQ}

Ground measurements  at point locations, $s$, within grid cell, $l$, country, $i$, region, $j$,  and  super--region, $k$  are denoted by $Y_{slijk}$. As described in Section \ref{sec:statsmod}, there is a nested hierarchical structure with $s=1,\dots, N_{lijk}$ sites within grid cell, $l$: $l=1,\dots, N_{ijk}$, grid cells within country $i$;  $i=1,\dots, N_{jk}$, countries within region  $j$: $j=1,\dots, N_k$,  regions  within super--region $k$: $k=1,\dots, N$.  In order to allow for the  skew in the measurements  and the constraint of non--negativity, the (natural) logarithm of the measurements are used.  \\



The model  consists of a set of fixed and random effects, for both intercepts and covariates, and is given as follows,
\begin{eqnarray} \label{eqn:arr1} \nonumber
\log(Y_{slijk}) = \beta_0 &+& \sum_{p_1 \in P_1} \beta_{p_1} X_{p_1,slijk} +\sum_{p_2 \in P_2} \beta_{p_2} X_{p_2,lijk}\\  \nonumber
&+& (\beta_{0, lijk}^G+ \beta_{0, ijk}^C+\beta_{0,jk}^R+\beta_{0,k}^{SR}) \\
&+& \sum_{q \in Q}(\beta_{q,ijk}^C+ \beta_{q,jk}^R+\beta_{q,k}^{SR}) X_{slijk} \\ \nonumber
&+& \epsilon_{slijk} \;.
\end{eqnarray}
Here, the set of $R$ covariates consists of two groups, $R=(P, Q)$, where $P$ are those with just  fixed effects and $Q$ those additionally assigned random effects. Within the group of $P$ fixed covariates, $P=(P_1, P_2)$, $P_1$ are measured at the locations of the ground monitors and $P_2$ are available at the level of the grid cell. The   term $\beta_{0,lijk}^G$ represents the intercept for grid cell $l$ that lies within country $i$, region $j$ and super--region $k$, with $\beta_{0,ijk}^C$, $\beta_{0,jk}^R$ and $\beta_{0k}^{SR}$ representing the corresponding intercepts for the country, region and super-region within this hierarchy. For the covariate effects, the notation is the same but there is no grid cell effect, with  $\beta_{q,ijk}^C$, $\beta_{q,jk}^R$ and $\beta_{q,k}^{SR}$ representing country, region and super--region effects respectively. The term $\epsilon_{slijk}$ denotes random error term with $\epsilon_{slijk} \sim N(0, \sigma^2_{\epsilon})$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Structure of the random effects}

Dropping the distinction between fixed-effect covariates  at point and grid cell level for clarity and expressing Equation (\ref{eqn:arr1})  in a similar form as that seen in Equation (\ref{eqn:3}) gives,
\begin{eqnarray} \label{eqn:arr1} \nonumber
\log(Y_{slijk}) = \tilde{\beta}_{0,lijk} &+& \sum_{q \in Q} \tilde{\beta}_{q, ijk} X_{q,slijk} \\ \nonumber 
&+& \sum_{p \in P} \beta_p X_{p,slijk}  \\
&+& \epsilon_{slijk} \;, 
\end{eqnarray}
where $\epsilon_{slijk} \sim N(0,\sigma_{\epsilon}^2)$ is a random error term.   \\

Here,  the random effect terms, $\tilde{\beta}_{0,lijk}$ and $\tilde{\beta}_{1,ijk}$, have contributions from  the country, the region and the super--region, with the intercept also having a random effect for the cell representing within-cell variation in ground measurements,  
\begin{eqnarray} \nonumber
\tilde{\beta}_{0, lijk} &=& \beta_0+ \beta_{0,lijk}^G + \beta_{0,ijk}^C + \beta_{0,jk}^R +\beta_{0,k}^{SR} \\ \nonumber
\tilde{\beta}_{q, ijk} &=& 	 \beta_q+  \beta_{q,ijk}^C + \beta_{q,jk}^R +\beta_{q,k}^{SR} \; .
\end{eqnarray}
For clarity of exposition, we restrict the following description to a generic parameter, $\beta$. Let $\beta^{SR}_k$ denote the coefficient for  super-region $k$. The coefficients for super-regions  are distributed with mean equal to the overall mean ($\beta_0$, the fixed effect) and variance, $\sigma_{SR}^2$, representing between super-region variability,
\begin{equation*}
\beta^{SR}_{k} \sim N(\beta_0,\sigma_{SR}^2) \,
\end{equation*}
where $k=1,\ldots,N = 7$. Similarly, each super-region contains a number of regions. Let $\beta^{R}_{jk}$ denote the coefficient for region $j$ (in super--region $k$) that will be distributed with mean equal to to the coefficient for the  super-region and variance representing the between region (within super--region) variability. 
\begin{equation*}
\beta^{R}_{jk} \sim N(\beta^{SR}_k,\sigma^2_{R,k}) 
\end{equation*}
where $j=1,\ldots,N_k$,  the number of regions in super-region $j$. Each region will  contain a number of countries. Let $\beta^{C}_{ijk}$ denote the coefficient for  country $i$ in region $j$ and super-region $k$. The country level effect will be distributed with mean equal  to the coefficient for region $j$ within super-region $k$ with variance representing  the between country (within region) variability.
\begin{equation} \label{eqn:countr1}
\beta^{C}_{ijk} \sim N(\beta^{R}_{jk},\sigma^2_{C, jk})
\end{equation}
where $i=1,\ldots,N_{jk}$ is   the number of countries in region $j$ (in super--region $k$). Note that in the case of the intercepts, there is an additional term, $\beta^G_{lijk}$,  representing between monitoring location, within grid cell, variability. \\

Country effects within regions and regional effects within super--regions  are assumed to be independent  within their respective geographies. However, the geographical hierarchy is broadly based on geographic regions, sub-continents, mortality and economic factors \citep{brauer2012exposure} and, as such, there are countries for which the allocation may not be optimal  when considering environmental factors, such as air pollution. For example, Mongolia is included within the Asia Central region and Central Eastern Europe and Central Asia super--region (see Figure \ref{map:regions}) but it's pollution profile might be expected to be more similar to its more direct neighbours, including China  (which is in a different region (Asia East) and super--region (South East Asia, East Asia and Oceania), rather than more western countries. For this reason, it might be advantageous to allow the borrowing of information in Equation (\ref{eqn:countr1}) to inlcude countries that are immediate neighbours rather than all of the countries in the surrounding administrative region. This could be achieved using a conditionally autoregressive (ICAR) model \citep{besag1974spatial} in place of Equation (\ref{eqn:countr1}), 
\begin{equation} \label{eqn:countr2}
\beta^{C}_{i} | \beta^{C}_{i'}, \; i' \in \partial_i \sim N\left(
  \overline{\beta}^{C}_{i},\frac{\psi^2}{N_{\partial i}}\right),
  \end{equation}
where $\partial i$ is the set of neighbours of country $i$, $N_{\partial i}$ is the number of neighbours, and $\overline{\beta}^{C}_i$ is the mean of the spatial random effects of these neighbours.

\subsection{Inference}
The model presented in Section \ref{sec:DIMAQ} is set within a Bayesian hierarchical framework that comprises of three main components: (i) the data, or observation level; (ii) the process, or parameter, level and (iii)  the hyperparameter level. 

\begin{eqnarray} \label{eqn:lgm1} \nonumber
\mbox{Data level: }\; Y_1, \dots, N_s|\theta, \psi &\sim& \prod^{N_S}_{s} p(Y_s| \theta, \psi)\\  \nonumber
\mbox{Parameter level: }\; \theta | \psi &\sim & p(\theta | \psi)\\
\mbox{Hyperparameter level: }\; \psi &\sim& p(\psi)
\end{eqnarray}
where $\theta$ are the parameters of the model as described in Section \ref{sec:DIMAQ} and will include \newline $\beta_0, \beta_{0,lijk}^G, \beta_{0,ijk}^C, \beta_{0,jk}^R, \beta_{0,k}^{SR}, \beta_q,   \beta_{q,ijk}^C,  \beta_{q,jk}^R$ and $\beta_{q,k}^{SR}$. The set of hyperparameters, $\psi$, contain those at both the first, $\psi_1$, and second, $\psi_2$ levels of the model, $\psi=(\psi_1, \psi_2)$, where $\psi_1=(\sigma^2_{\epsilon})$ and $\psi_2=(\sigma^2_{G,i},\sigma^2_{C,j}, \sigma^2_{R,j}, \sigma^2_{SR})$. \\


The model is implemented using approximate Bayesian inference using integrated nested Laplace Approximations (INLA) proposed in \citet{rue2009approximate} using the R-INLA software \citep{rue2012r}. R-INLA can be used with models that can be expressed as a latent Gaussian model (LGM). 

\subsubsection{Latent Gaussian models}
The model presented in Section \ref{sec:DIMAQ} can be expressed in terms of an LGM meaning that we can take advantage of features that can facilitate efficient computation. LGMs  are a general class of models and allow a very wide range of formulations.  Given $\eta_s = g(E(Y_s))$, where  $g()$ is a link function, the general form  of an LGM is

\begin{eqnarray}
\eta_s &=& \beta_0 + \sum_{p=1}^{P} \beta_p X_{qs} + \sum^Q_{q=1} f_q (Z_{qs}) 	
\end{eqnarray}
where $\beta_0$ is an overall intercept term, the set of $\beta_p$ $(p=1,\dots, P)$ are the coefficients associated with covariates, $X$; the fixed effects. The set of functions,  $f_1(\cdot), \dots, f_Q(\cdot)$ represent the random effects with the form of the function being determined by the model. For example a hierarchical model may have, $f_1(\cdot) \sim N(0, \sigma^2_f)$, with a distribution defined for $\sigma^2_f$, whereas for standard regression, $f(\cdot) \equiv 0$, leaving just fixed effects. \\

The set of unknown parameters, $\theta$, will include both the coefficients of the model shown above and the parameters required for the functions, i.e. $\theta = (\beta_p, f_q)$. For an LGM, the collection of all of these parameters will be assigned a Normal distribution  in the second level of the model shown in Equation (\ref{eqn:lgm1}), e.g. $\theta | \psi \sim  MVN(\theta | \Sigma(\psi_2))$. The computation required to perform inference on an LGM will be largely determined by the characteristics of the covariance matrix, $\Sigma (\psi_2)$. This will often be dense, i.e. it will have many entries that are non-zero, which commonly leads to a high computational burden when performing  the matrix inversions that will be required to perform inference. \\

If  $\theta | \psi$ can be expressed in terms of a Gaussian Markov Random Field (GMRF),  then it may be possible to take advantage of methods that reduce computation when performing Bayesian analysis on models of this type \citep{rue2005gaussian}. Using a GMRF means that   typically  the inverse of the covariance matrix, $Q = \Sigma^{-1}$ will be sparse, i.e. more zero entries,  due to the conditional independence between sets of parameters in which $\theta_l \ci  \theta_m | \theta_{-lm} \iff Q_{lm}=0$ (where $-lm$ denotes the vector of $\theta$ with the $l$ and $m$ elements removed) \citep{rue2005gaussian}. Expressing  Equation (\ref{eqn:lgm1}) in terms of the precision, rather than the covariance, gives $\theta | \psi \sim  MVN(\theta | Q(\psi_2)^{-1}$), where  $\psi_2$  denotes the parameters associated with $Q$ rather than $\Sigma$. \\

\subsubsection{Integrated Laplace Approximations}

Estimation of the (marginal) distributions of the model parameters and hyperparameters of the LGM shown in Equation (\ref{eqn:lgm1}) will require evaluation of the following integrals:

\begin{eqnarray} \nonumber \label{eqn:lgm2}
	p(\theta_j | Y) &=& \int p(\theta_j | Y, \psi)p(\psi|Y) d \psi \\ 
		p(\psi_k | Y) &=& \int p(\psi | Y) d \psi_{-k}
\end{eqnarray}

In all but the most stylised cases, these will not be analytically tractable. Samples from these distributions could be obtained using Markov-chain Monte Carlo methods but  there may be issues when fitting complex LGMs and the computational burden may be excessive, especially large numbers of predictions are required.   Here,   approximate Bayesian inference is performed  using INLA. It is noted that the dimension of $\theta$ is much larger than the dimension of $\psi$ and this will help in the implementation of the model as the computational burden increases linearly with the dimension of $\theta$ but exponentially with the dimension of $\psi$.\\



The aim is to find approximations for the distributions shown in Equation (\ref{eqn:lgm2}).  For the hyperparameters, the posterior of $\psi$ given $Y$ can be written as

\begin{eqnarray} \nonumber
p(\psi|Y) &=& \frac{p(\theta,\psi| Y)}{p(\theta| \psi, Y)} \\ \nonumber
&\propto & \frac{p(Y|\theta)p(\theta|\psi)p(\psi)}{p(\theta|\psi, Y)} \\  \nonumber
&\approx & \left.\frac{p(Y|\theta)(\theta|\psi)p(\psi)}{\tilde{p}(\theta|\psi, Y)} \right| _{\theta = \hat{\theta}(\psi)} \\ 
&=& \tilde{p}(\psi | Y)\; .
\end{eqnarray}
Here a Laplace approximation (LA) is used in the denominator for $\tilde{p}(\theta|\psi, Y)$. For univariate $\theta$ with an integral of the form $\int e^{g(\theta)}$, the LA takes the form $g(\theta) \sim N(\hat{\theta}(\psi), \hat{\sigma}^2)$, where $\hat{\theta}(\psi)$ is the modal value of $\theta$ for specific values of the hyperparameters, $\psi$ and $\hat{\sigma}^2 = \left\{ \frac{d^2 \log g(\theta)}{d \theta^2} \right \}^{-1}$. \\

The mode of $\tilde{p}(\psi | Y)$ can be found numerically by Newton type algorithms. Around the mode, the  distribution, $\log \tilde{p} (\psi | Y)$, is evaluated over a grid of $H$ points,  $\{\psi^*_h\}$, with  associated integration weights $\Delta_h$.  For each point on the grid, the marginal posterior, $\tilde{p}(\psi_h^* | Y)$ is obtained from which approximations to the marginal distributions,  $\tilde{p}(\psi |Y)$, can be found using numerical integration. \\


For the model individual model parameters, $\theta_j$,

\begin{eqnarray} \nonumber
p(\theta_j|Y) &=& \frac{p((\theta_j, \theta_{-j}),\psi| Y)}{p(\theta_{-j}| \theta_{j}, \psi, Y)} \\ \nonumber
&\propto & \frac{p(Y|\theta)p(\theta|\psi)p(\psi)}{p(\theta_{-j}| \theta_{j}, \psi, Y)}\\ 
&\approx & \left.\frac{p(Y|\theta)(\theta|\psi)p(\psi)}{\tilde{p}(\theta_{-j}| \theta_{j}, \psi, Y)} \right| _{\theta_{-j} = \hat{\theta_{-j}}(\theta_{j}, \psi)} \\ \nonumber
&=& \tilde{p}(\theta_j | \psi, Y)\; .
\end{eqnarray}

For an LGM, $(\theta_{-j}| \theta_{j}, \psi, Y)$ will be approximately Gaussian. There are a number of ways of constructing the approximation in the denominator including a simple Gaussian approximation which will be   computationally attractive but may be inaccurate. Alternatively, a LA would be  highly accurate but computationally expensive. R-INLA uses a computationally efficient method,  a simplified LA, that consists of performing a Taylor expansion around the LA of $\tilde{p}(\theta_j|\psi, Y)$, aiming to
`correct' the Gaussian approximation for location and
skewness \citep{rue2009approximate}.\\

The marginal posteriors, $\tilde{p}(\psi^*_h | Y)$, that have been evaluated at points $h^*$, are used to obtain the conditional posteriors,  $\tilde{p}(\theta_j | \psi^*_h, Y)$, on a grid of values for $\theta_j$. The marginal posteriors, $\tilde{p}(\theta_j |  Y)$, are then found by  numerical integration: $\tilde{p}(\theta_j |  Y) = \sum^H_h = \tilde{p}(\theta_j | \psi^*_h, Y)\tilde{p}(\psi^*_h|Y) \Delta_h$, with the integration weights, $\Delta_h$ being  equal when the grid takes the form of a regular lattice. \\

The model presented in Section \ref{sec:DIMAQ}  was implemented using  R-INLA  \citep{rue2012r} using the Balena high performance computing system (HPC) at the the University of Bath \newline \verb (www.bath.ac.uk/bucs/services/hpc/facilities/).  Fitting the model described in Section \ref{sec:DIMAQ} to data from the 6003 monitors (and associated covariates) does not itself require the use of an HPC but the prediction on the entire grid (of 1.4 million cell) did present some computational challenges.  INLA requires a copy of the model to be stored on a single  node which,  even with the high-memory compute nodes (32GBs per core) available with the HPC, resulted in memory issues when attempting to perform estimation and prediction on the entire grid in one step. Therefore, an iterative approach to prediction was used, repeatedly appending subsets of the prediction grid (with associated data on satellite estimates and other predictors)  to the modelling dataset,  until a complete set of global predictions  were obtained.



==> Sections/4_results_20160817_MLT.tex <==
\section{Results}

A series of models based on the structure described in Section \ref{sec:DIMAQ} were applied with the aim of assessing the predictive ability of potential explanatory factors. The choice of which variables were included in the model was made based on their contribution to within-sample model fit and out-of-sample predictive ability.  \\
 
In addition to four models based on that shown in  Equation (\ref{eqn:arr1}), the results of fitting the model used in GBD2013 \citep{brauer2015exposure} (model (i)) are given for comparison. This is a  linear regression model with response equal to the average concentration from monitors within a grid cell and covariates $X_1, X_2$ and $X_3$ together with the  average of the satellite based estimates and those from the TM5-FASST chemical transport model for each cell, $(X_4+X_5)/2$. \\
 
Details of the variables included in five candidate models can be see in Table \ref{tab:models} They include information on local network characteristics; whether the type of monitor was unspecified, $X_1$; whether the exact location is known, $X_2$, and whether PM$_{2.5}$ was estimated from PM$_{10}$ ($X_3$); satellite based estimates of PM$_{2.5}$ concentrations ($X_4$),  estimates of PM$_{2.5}$ ($X_5$),  dust ($X_6$) and the sum of sulphate, nitrate, ammonium and organic carbon ($X_7$) from atmospheric models;  estimates of  population ($X_8$) and a function of land--use and elevation ($X_9$).  Except for the measurements themselves, all of these variables  are spatially aligned to the resolution of the  grid. Further details  can be found in Section \ref{sec:data}. \\ 
 
For evaluation, cross validation was performed using 25 combinations of training (80\%) and validation (20\%) datasets.  Validation sets were obtained by taking a stratified random sample, using sampling probabilities based on the cross-tabulation of PM2.5 categories (0-24.9, 25-49.9, 50-74.9, 75-99.9, 100+ $\mu$gm$^{-3}$) and super-regions, resulting in concentrations in each validation sets having the same distribution of PM2.5 concentrations and super-regions as the overall set of sites.  The following metrics were calculated for each training/evaluation set combination: for model fit: R2 and deviance information criteria (DIC, a measure of model fit for Bayesian models) and for predictive accuracy:  root mean squared error (RMSE) and population weighted root mean squared error (PwRMSE).\\ 

\begin{table}[hbt]
\centering
  \begin{tabular}{ccccccccccc}
{\bf Model} &\multicolumn{2}{c}{\bf  (i)}  &\multicolumn{2}{c}{\bf  (ii)} 
 & \multicolumn{2}{c}{\bf  (iii)}  &\multicolumn{2}{c}{\bf  (iv)}
  &\multicolumn{2}{c}{\bf  (v)}\\
 Variable & F & R & F & R& F & R& F & R& F & R \\
    \hline
   Intercept &   \checkmark & &\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark \\
    $X_1^{\dagger}$ &   \checkmark & &\checkmark&&\checkmark&&\checkmark&&\checkmark\\
    $X_2^{\dagger}$ &   \checkmark & &\checkmark&&\checkmark&&\checkmark&&\checkmark\\
    $X_3^{\dagger}$ &   \checkmark & &\checkmark&&\checkmark&&\checkmark&&\checkmark\\
$X_4$ &   \checkmark & &\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark \\
$X_5$ &   \checkmark & &&&\checkmark&\checkmark&&&\checkmark&\checkmark \\
$X_6$ &   & &&&&&\checkmark&\checkmark&\checkmark&\checkmark \\
$X_7$ &   & &&&&&\checkmark&\checkmark&\checkmark&\checkmark \\
$X_8^{\dagger\dagger}$ &    & &\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark\\
$X_9$ &   & &&&&&\checkmark&\checkmark&\checkmark&\checkmark \\
    \hline\\
 \multicolumn{11}{l} {    $\dagger$ Together with interaction with $X_4$, $X_5$ where they are}\\  \multicolumn{11}{l} {  included within the model. }\\
\multicolumn{11}{l} { $\dagger\dagger$ Country level random  
effects are assigned a}\\
 \multicolumn{11}{l} {conditional autoregressive prior.}
  \end{tabular}
  \caption{Variables includes in each of five candidate models: $X_1$, whether the type of monitor was unspecified; $X_2$, whether the exact location is known; $X_3$, whether PM$_{2.5}$ was estimated from PM$_{10}$;  $X_4$, satellite based and $X_5$ chemical transport model estimates of PM$_{2.5}$; $X_6$ and $X_7$, estimates of compositional concentrations of mineral dust and the sum of sulphate, nitrate, ammonium and organic carbon from atmospheric models; $X_9$, a function of elevation difference and land--use. See text for details.} \label{tab:models}
\end{table}

 The results of fitting the five candidate models can be seen in Table \ref{tab:tab1}, which shows     R$^2$ and Deviance Information Criteria (DIC) for within sample model fit and  root mean squared error (RMSE) and population weighted root mean squared error (PwRMSE) for out-of-sample predictive ability, and Figure \ref{fig:res1} which shows the PwRMSE for each model by super-region. It can be seen that using any of the hierarchical model described in Section \ref{sec:DIMAQ} provide an immediate improvement in all metrics when compared to the linear model, with a single global calibration function, used in GBD2013. For example, using model (ii) which contains satellite based estimates, population and local network characteristics  results in the overall $R^2$ improving from 0.54 to 0.90, DIC from 7828 to 1105 and reductions of  5.9 and 10.1 $\mu$gm$^{-3}$ for RMSE and population weighted RMSE respectively. This improvement can be seen in each of the super-regions (Figure \ref{fig:res1}), with the most marked improvements in areas where there is limited ground monitoring. \\  
 
 Adding either estimates of PM$_{2.5}$ from the TM5-FASST chemical transport model (model iii) or estimates of specific chemical components and dust from the GEOS-Chem chemical transport model together with and information on differences in elevation between a ground monitor and its surrounding grid cell (model iv) to this resulted in further improvements with model (iii) showing the most improvement. Adding the estimates of PM$_{2.5}$ from the TM5-FASST chemical transport model to model (iv) did not result in any substantial improvement in  predictive ability. This may be in part due to the fact that the variables used in model (iv) are produced for 2014 whereas the estimates from the TM5-FASTT model are from 2010. Considering the lack in improvement of predictive ability and the increased complexity and computational burden involved when incorporating an additional set of random effects, these estimates are not therefore not included in the final model (model (iv)).  \\

\begin{table}[h]
\centering
\begin{footnotesize}
\begin{tabular}{clllll}
\multicolumn{1}{c} {\bf Model} & \multicolumn{1}{c} {\bf R$^2$} & \multicolumn{1}{c} {\bf DIC} & \multicolumn{1}{c} {\bf RMSE$\dagger$} & \multicolumn{1}{c} {\bf PwRMSE$\dagger$} \\
\hline 
(i) & 0.54 (0.53, 0.54)& 7828 (7685, 8657)& 17.1 (16.5, 18.1)&  23.1 (20.5, 29.3)\\
(ii) & 0.90 (0.90, 0.91)& 1105 (849, 1239)& 11.2 (10.1, 12.9)& 13.0 (11.5, 23.5)\\
 (iii) & 0.90 (0.90, 0.91)& 986 (704, 1115)& 11.1 (10.0, 13.3)& 12.8\ (11.2, 23.0)\\
 (iv) & 0.91 (0.90, 0.91)& 877 (640, 1015)& 10.7 (9.5, 12.3)& 12.1 (10.7, 21.4)\\
 (v) & 0.91 (0.90, 0.92)& 777 (508, 919) & 10.7 (9.5, 12.5)& 12.0 (10.7, 20.7)\\
\hline 
$\dagger \; \mu$gm$^{-3}$
\end{tabular}
\end{footnotesize}
\caption{Summary of results from fitting five candidate models. Model  (i) is the model used in the GBD2013 study. Model (ii) is a   hierarchical model containing satellite based estimates of PM$_{2.5}$, population and  local network characteristics. Models (iii-v) contain  additional variables:  model (iii),     estimates  of PM$_{2.5}$ from   the TM5-FASST chemical transport  model;  model (iv),   estimates of specific chemical components and dust from the GEOS-Chem chemical transport model and information on differences in elevation between a ground monitor and its surrounding grid cell (as defined by the GEOS-Chem chemical transport model); (v)  both the estimates from the TM5-FASST and GEOS-Chem  models.  See text for further details. Results are for both in-sample model fit and out-of-sample predictive ability and  are the median (minimum, maximum) values from 25 training-validation set combinations. For  within sample model fit,   R$^2$ and Deviance Information Criteria (DIC).  For out-of-sample predictive ability, root mean squared error (RMSE) and population weighted root mean squared error (PwRMSE). } \label{tab:tab1}
\end{table}


 
  \begin{figure}
 \centering
 \includegraphics[scale=0.5]{Figures/PopRMSE_by_SRegion.pdf}	
 \caption{Summaries of predictive ability of the GBD2013 model (i) and four candidate models (ii-iv), for each of seven super--regions: 1, high income; 2, Central Europe, Eastern Europe, Central Asia; 3, Latin America and Caribbean; 4, Southeast Asia, East Asia and Oceania; 5, North Africa / Middle East; 6, Sub-Saharan Africa; 7, South Asia. For each model,  population weighted root mean squared errors ($\mu$gm$^{-3}$) are given with dots denoting the median of the distribution from 25 training/evaluation sets and the vertical lines the range of values.} \label{fig:res1}
 \end{figure}

Predictions from the final model (model (iv)) can be seen in Figures \ref{map:pred} and \ref{map:ci}. The point estimates shown in Figure \ref{map:pred} give a summary of air quality for each  grid cell and show clearly the spatial variation in global PM$_{2.5}$. For each grid cell, there is an underlying (posterior) probability distribution which incorporates information about the uncertainty of these estimates. There are a number of ways of presenting this uncertainty and Figure \ref{map:ci} shows one of these; half of the length of the 95\% credible intervals \citep{denby2007uncertainty}. Higher uncertainty will be combination of higher concentrations and sparsity of monitoring data and the effects of these can be clearly seen in areas of North Africa and the Middle East. \\
 
 The distributions for each cell can also be used to examine the probabilities of exceeding particular thresholds. Figure \ref{map:china} shows an example of this and contains predicted concentrations for China (Figure \ref{map:china1}) together with the probability for each cell that the value exceeds 35 $\mu$gm$^{-3}$ (Figure \ref{map:china2}) and 75 $\mu$gm$^{-3}$ (Figure \ref{map:china3}). High probabilities of exceeding the greater of the two thresholds are observed in the area around Beijing and in the Xinjiang province in the far west of the country. For the latter,  a substantial component of the high (estimated) concentrations  will  be  due to mineral dust from the  large deserts in the region, as can be seen in Figure \ref{map:ctm3}. The distribution of estimated exposures shown in the map of median values (of the posterior distributions) shown in Figure \ref{map:china1} can also be seen in Figure \ref{map:milliegram1}  which suggests three distinct properties of air pollution (PM$_{2.5}$) in this country: (i) a land mass with low levels of air pollution; (ii) a much larger proportion of the total land mass with (comparatively) high levels; and (iii) a substantial area with very high levels. In terms of potential risks to health, it is high levels in areas of high population that will drive the disease burden. Figure \ref{map:milliegram2} shows the distribution of estimated population level exposures, calculated by multiplying the estimate in each grid cell by its population. It can seen that only a small proportion of the population reside in areas with the lowest concentrations of PM$_{2.5}$ with vast the majority of the population experiencing high and very high levels of PM$_{2.5}$. 
  
 
  \begin{figure} 
 \centering
 \begin{subfigure}{\textwidth}  \centering
 \includegraphics[width=0.8\linewidth]{Figures/world_pred_2014.png}
 \caption{Medians of  posterior distributions.} 
 \label{map:pred}
 \end{subfigure}
  \begin{subfigure}{\textwidth}  \centering
 \includegraphics[width=0.8\linewidth]{Figures/world_halfCI_2014.png}
 \caption{Half the width of  95\% posterior credible intervals.} \label{map:ci}
 \end{subfigure} 
 \caption{Estimates of annual averages of PM$_{2.5}$ ($\mu$mg$^{-3}$) for 2014 together with  associated uncertainty for each grid cell ($0.1^o \times 0.1^o$ resolution) using a Bayesian hierarchical model (see text for details).}
 \end{figure}  
  
  
  
    \begin{figure} 
 \centering
 \begin{subfigure}{\textwidth}  \centering
 \includegraphics[width=0.6\linewidth, clip=TRUE, trim = {0 10mm 0 18mm}]{Figures/china_pred_2014.png}
 \caption{Medians of  posterior distributions.} 
\label{map:china1}
 \end{subfigure}
  \begin{subfigure}{\textwidth}  \centering
 \includegraphics[width=0.6\linewidth, clip=TRUE, trim = {0 10mm 0 18mm}]{Figures/china_prob35.png}
 \caption{Probability of  exceeding 35 $\mu$gm$^{-3}$.} 
 \label{map:china2}
 \end{subfigure} 
  \begin{subfigure}{\textwidth}  \centering
 \includegraphics[width=0.6\linewidth, clip=TRUE, trim = {0 10mm 0 18mm}]{Figures/china_prob75.png}
 \caption{Probability of  exceeding 75 $\mu$gm$^{-3}$.}
 \label{map:china3}
 \end{subfigure} 
 \caption{Estimates of annual mean PM$_{2.5}$ concentrations ($\mu$mg$^{-3}$) for 2014 together with  exceedance probabilities using a Bayesian hierarchical model (see text for details) for each grid cell ($0.1^o \times 0.1^o$ resolution) in China.}
 \label{map:china}
 \end{figure}  
  
 \begin{figure} 
 \centering
 \begin{subfigure}{0.47\textwidth}  \centering
 \includegraphics[width=\linewidth]{Figures/china_hist1_2014.pdf}
 \caption{Estimated annual average concentrations of PM$_{2.5}$ by grid cell ($0.1^o \times 0.1^o$ resolution). Black crosses denote the annual averages recorded at ground monitors.}
\label{map:milliegram1}
 \end{subfigure}\hspace{5pt}
  \begin{subfigure}{0.47\textwidth}  \centering
 \includegraphics[width=\linewidth]{Figures/china_hist2_2014.pdf}
 \caption{Estimated population level exposures (blue bars) and, for cells containing at least one monitoring station,   population weighted measurements from ground monitors (black bars). } 
 \label{map:milliegram2}
 \end{subfigure} 
 \caption{Distributions of annual mean concentrations  and population level exposures for PM$_{2.5}$ ($\mu$mg$^{-3}$) in China.}
 \label{map:milliegram}
 \end{figure}  
  
  
  

  

